Time to augment self-supervised visual representation learning

Biological vision systems are unparalleled in their ability to learn visual representations without supervision. In machine learning, self-supervised learning (SSL) has led to major advances in forming object representations in an unsupervised fashion. Such systems learn representations invariant to augmentation operations over images, like cropping or flipping. In contrast, biological vision systems exploit the temporal structure of the visual experience during natural interactions with objects. This gives access to "augmentations" not commonly used in SSL, like watching the same object from multiple viewpoints or against different backgrounds. Here, we systematically investigate and compare the potential benefits of such time-based augmentations during natural interactions for learning object categories. Our results show that time-based augmentations achieve large performance gains over state-of-the-art image augmentations. Specifically, our analyses reveal that: 1) 3-D object manipulations drastically improve the learning of object categories; 2) viewing objects against changing backgrounds is important for learning to discard background-related information from the latent representation. Overall, we conclude that time-based augmentations during natural interactions with objects can substantially improve self-supervised learning, narrowing the gap between artificial and biological vision systems.

==> Time To Augment Contrastive Learning – ICLR23/content.tex <==
\section{Introduction}

%Babies recognize categories before being able to name objects \cite{quinn1993evidence}, suggesting that they perform unsupervised object recognition. Similarly to babies, l
Learning object representations without supervision is a grand challenge for artificial vision systems. Recent approaches for visual self-supervised learning (SSL) acquire representations invariant to data-augmentations based on simple image manipulations like crop/resize, blur or color distortion \citep{grill2020bootstrap,chen2020simple}. The nature of these augmentations determines what information is retained and what information is discarded, and therefore how useful these augmentations are for particular downstream tasks \citep{jaiswal2021survey,tsai2020self}.
%
Biological vision systems, in contrast, appear to exploit the temporal structure of visual input during interactions with objects for unsupervised representation learning. According to the slowness principle \citep{wiskott2002slow, li2010unsupervised, wood2018development}, biological vision systems strive to discard high-frequency variations (e.g.\ individual pixel intensities) and retain slowly varying information (e.g.\ object identity) in their representation. Incorporating this idea into SSL approaches has led to recent time-contrastive learning methods that learn to map inputs occurring close in time onto close-by latent representations \citep{oord2018representation,schneider2021contrastive}.
%It follows that time-based visual augmentations result from how humans interact with the environment, in particular during the critical period of object understanding in infants \cite{smith2018developing}.
% New sentences from Jochen:
How these systems generalize depends on the temporal structure of their visual input. In particular, visual input arising from embodied interactions with objects may lead to quite different generalizations compared to what is possible with simple image manipulations.
%https://www.overleaf.com/project/62680c60c1bb74fc797df530
For instance, human infants learning about objects interact with them in various ways \citep{smith2018developing}.
%, which will determine what aspects of the visual input vary slowly vs.\ quickly.
%First, they execute saccadic eye movements and accommodate their pupils to the distance of the fixation point. This enables them to keep object features in focus while blurring background features due to their limited depth of field. 
First, infants rotate, bring closer/farther objects while playing with them \citep{byrge2014developmental}. Second, as they gain mobility, they can move in the environment while holding an object, viewing it in different contexts and against different backgrounds. We refer to (simulations of) such interactions as {\em natural interactions}. %Third, while moving an object, different levels of lights may be reflected on it, modifying its perceived color. %The constant change of illuminations/light colors coming from both the sun/sky or artificial light further increases the overall set of experienced color changes \cite{gilchrist1999anchoring}. 

Here, we systematically study the impact of such natural interactions on representations learnt through time-contrastive learning
%. To simulate the interactions available to an infant, we investigate time-based augmentations
in \rebut{different} settings. We introduce two new simulation environments based on the near-photorealistic simulation platform ThreeDWorld (TDW) \citep{gan2021threedworld} and combine them with a recent dataset of thousands of 3D object models (Toys4k) \citep{stojanov2021using}.
\rebut{Then} we validate our findings on two video datasets of \rebut{real human object manipulations}, ToyBox
%validates the importance of object manipulations
\citep{wang2018toybox} and
% we systematically study with
CORe50 \citep{lomonaco2017core50}.
%the impact of relative frequencies of object manipulations and ego-motion on the learned representation. %and we dynamically re-segment real-world videos of object manipulations from the CORe50 dataset \citep{lomonaco2017core50} to approximate different types of natural interactions and systematically study the impact of relative frequencies of the interactions on the learned representation. 


% ME There has to be one sentence about combining both approaches where we can again use the phrase augment contrastive learning
%Our experimental contributions show that time-based augmentations derived from natural interactions consistently outperform the standard augmentation set \cite{chen2020simple} used in machine learning in categorizing unseen objects.
%, while performing at least as well on their own.
Our experiments show that adding time-based augmentations to conventional data-augmentations considerably improves category recognition. Furthermore, we show that the benefit of time-based augmentations \rebut{during natural interactions} has two \rebut{main} origins. First, 3-D object rotations boost generalization across object shapes. Second, viewing objects against different backgrounds while moving with them reduces harmful effects of background clutter.
%Furthermore, we note that the combination of saccades and distance changes of objects have a similar effect to the standard crop/resize augmentation. 
We conclude that exploiting natural interactions via time-contrastive learning greatly improves self-supervised visual representation learning.


%# which are more-or-less different from standard augmentations used in machine learning.

%On the biological side, several experiments suggest that humans learn visual representation using the slowness principle \cite{li2010unsupervised,wood2018development}, \textit{i.e}, they discard  According to this hypothesis contrastive learning become a plausible way to implement the slowness principle as we consider

%The idea is that an image and its augmented variant should be similar in a learnt representation space, and dissimilar to other images. 

%On the biological side, several experiments suggest that humans learn visual representation using the slowness principle \cite{li2010unsupervised,wood2018development}, \textit{i.e}, they discard high-frequency varying information and extract slowly moving features in their internal representation. According to this hypothesis contrastive learning become a plausible way to implement the slowness principle as we consider

%Paragraph on self-supervised learning and data augmentations

%Explain they are unrealistic

%Contribution: introduction of realistic data-augmentations


\section{Related work}

% \paragraph{SimCLR-TT.} SimCLR is a recent state-of-the-art, unsupervised, CL approach that manages to learn visual representations suitable to downstream tasks \citep{chen2020simple}. The general idea is that two semantically close/different inputs should be close/distant in the learnt representation space. The underlying assumption is that applying certain transformations does not change the semantic meaning or label of an image, and thus should only slightly change the representation of that image. They sample an image $i$, apply transformations to it taken from a predefined set of transformations, resulting in two new images $x_i$ and $x_j$, also called a positive pair. The same procedure is applied to a batch of $N-1$ sampled different images resulting in $2N-2$ images, also called negative samples. Its time-based variant, SimCLR-TT \citep{schneider2021contrastive, oord2018representation}, assumes that semantically close images are also close in time, such that $x_i$ and $x_j$ are successors in time. Then, both SimCLR and SimCLR-TT learn the parameters $\theta$ of the representation encoder (a neural network) $f_{\theta}$ to minimize:
% %
% \begin{equation}
%     \mathcal{L}_{i,j}= -\log \frac{e^{\text{sim}(f_{\theta}(x_i), f_{\theta}(x_j))/\tau}}{\sum_{k=1,k\neq i, k\neq j}^{2N} e^{\text{sim}(f_{\theta}(x_i), f_{\theta}(x_k))/\tau}}, \label{eq:simclr}
% \end{equation}
% %
% where \textit{sim} is a similarity function and $\tau$ is a temperature hyper-parameter. The numerator makes sure that positive pairs are close in the latent space. The denominator ensures that the image embeddings stay relatively distant from each other and do not collapse to a single point.

\paragraph{Data-augmented self-supervised learning.}
%Recent developments in self-supervised learning have been shown to successfully learn visual representations suitable to downstream tasks \citep{chen2020simple}.
The general idea \rebut{behind} most recent approaches \rebut{for self-supervised learning} is that two semantically close/different inputs should be \rebut{mapped to} close/distant \rebut{points} in the learnt representation space. \rebut{Applying a certain transformation to an image such as flipping it horizontally generates an image that will be very different at the pixel level, but has a similar semantic meaning. A learning objective for SSL will therefore try to ascertain that the representations of an image and its augmented version are close in latent space, while being far from the representations of other unrelated images.} 

%The underlying assumption is that applying certain transformations does not change the semantic meaning or label of an image, and thus should only slightly change the representation of that image. The
\rebut{A concrete} approach may work as follows: sample an image $x$, apply transformations to it taken from a predefined set of transformations, resulting in new images $x'$, also called a positive pair. The same procedure is applied to a batch of different images.
%The initial and positive images are embedded through a Siamese-like architecture.
Embeddings of positive pairs are brought together while keeping the embeddings of the batch overall distant from one another. There are three main categories of approaches \rebut{for doing so}: contrastive learning methods \citep{chen2020simple,he2020momentum} explicitly push away the embeddings of a batch of inputs from one another; distillation-based methods \citep{grill2020bootstrap,chen2021exploring} use an asymmetric embedding architecture, allowing the model to discard the ``push away'' part; entropy maximization methods \citep{bardes2022vicreg,ermolov2020latent} \rebut{maintain} a high entropy \rebut{in the embedding space}.

%For our experiments we consider the SimCLR \citep{chen2020simple}, as well as VICReg \citep{bardes2022vicreg} and BYOL \citep{guo2020bootstrap} algorithms to provide a state of the art foundation to our experiments.

% \paragraph{Time-contrastive learning in reinforcement learning.}

% Recent studies investigated time-contrastive learning in a reinforcement learning (RL) setting, but unlike this work, they do not consider realistic interactions with objects. The learnt time-contrastive representations are used in several ways: as an auxiliary task to speed up the extraction of interested features \cite{oord2018representation,laskin2020curl}; to pre-train a representation for RL \cite{stooke2021decoupling}; to provide rewards in imitation learning settings \cite{sermanet2018time}; to generate intrinsic rewards for improving the exploration of agents \cite{guo2021geometric,yarats2021reinforcement} or learning skills \cite{li2021learning,aubret2021distop,nachum2019near}; to perform model-based reinforcement learning in latent space \cite{okada2021dreaming}. Other approaches also consider action-aware variant of time-contrastive learning \cite{schwarzer2020data, shu2020predictive, nachum2019near}. In fact, by keeping the information in the observation that is impacted by actions, the learnt representation may be optimal to solve a RL task \cite{rakelly2021mutual}. It is also possible to apply a time-contrastive loss in a multi-scale fashion on the filters of a convolutional neural network (CNN) \cite{anand2019unsupervised}. We hope further work will explore the connection between actively learning task-useful representations and object-oriented representation.

%occlusion \cite{fong2019occlusions}
 \paragraph{\rebut{Image manipulations as} data-augmentations.} Most self-supervised learning approaches have used augmentations based on simple image manipulations to learn representations. Frequently used are color distortion, cropping/resizing a part of an image, the horizontal flipping of an image, gray scaling the image, and blurring the image \citep{chen2020simple}. Other augmentations can be categorized in three ways \citep{shorten2019survey, jaiswal2021survey}: 1) geometric augmentations include image rotations \citep{chen2020simple} or image translations \citep{shorten2019survey}; 2) Context-based augmentations include jigsaw puzzle augmentations \citep{noroozi2016unsupervised,misra2020self}, pairing images \citep{inoue2018data}, greyed stochastic/saliency-based occlusion \citep{fong2019occlusions,zhong2020random}, or automatically modifying the background \citep{ryali2021learning}. 3) Color-oriented transformations can be the selection of color channels \citep{tian2020makes} or Gaussian noise \citep{chen2020simple}. A related line of work also proposes learning how to generate/select data-augmentations \citep{cubuk2018autoaugment,tian2020makes}, but since it takes advantage of labels, the approach is no longer self-supervised. %We expect that actively selecting what to perceive, typical of how an infant interacts with objects \citep{james2001manipulating,smith2018developing}, will further improve the benefits of our natural augmentations.
 
 % search on data augmentations \cite{shijie2017research}
 
 \paragraph{Time-based data-augmentations.}
 Several works have proposed using the temporality of interactions to learn visual representations.
 %, but they consider smaller sets of interactions, uncontrolled natural interactions or do not apply it to solve category recognition.
 A recent line of work proposes to learn embeddings of video frames using the temporal contiguity of frames:
%  Some approaches propose to learn embeddings of video frames using the temporal contiguity of frames \cite{knights2021temporally, orhan2020self}. However, they do not analyze the impact of each interaction type, do not consider fundamental properties of vision such as a finite depth of field and datasets are restricted to few weeks of interactions.
 \citet{knights2021temporally} propose a learning objective that makes codes of adjacent frames within a video clip similar, however the system still needs to have information about where each video starts and ends. In contrast, our setups expose the system to a continuous stream of visual inputs.  \rebut{Other methods showed the importance of time-based augmentations based on videos for object tracking \citep{xu2021rethinking}, category recognition \citep{gordon2020watching,parthasarathy2022self,orhan2020self} or adversarial robustness \citep{kong2021models}. Unlike us they do not make an in-depth analysis of the impact of different kinds of natural interactions.} %and do not consider fundamental aspects of vision such as a finite depth of field. 
 %Frame similarity in videos has also been used for object tracking , or.
 % In contrast, our setups expose the system to a continuous stream of visual inputs.  much more like \citet{orhan2020self}. But instead of trying to segment the stream into temporal classes our approach focuses on the representation of object categories.
 %parthasarathy2022self
 %and datasets are restricted to few weeks of interactions.
\citet{schneider2021contrastive} showed the importance of \rebut{natural interactions with objects} for \rebut{learning} object \rebut{representations}, but only considered small datasets of few objects, without complex backgrounds and without studying generalization over categories of objects. \citet{wang2021use} have shown that one can replace crop augmentations by saccade-like magnifications of images, \rebut{establishing a link between conventional image-based and more natural time-based augmentations.}
%, but they use datasets of static images, making impossible to truly simulate a view change. \rebut{Saccades can induce peripheral/mid-level visual processing, which aids to learn robust representations in humans \citep{harrington2021finding}.}
\citet{aubret2022toddler} \rebut{studied the impact of embodiment constrains on object representations learnt through time-contrastive learning during natural interactions}. They highlight that complex backgrounds negatively impact the representations of objects. \rebut{Here} we show that allowing the agent to move with objects so that they are seen against changing backgrounds improves robustness against background complexity.
 
 \rebut{We note that} a large body of work also considers time-contrastive learning in the context of reinforcement learning \citep{oord2018representation,laskin2020curl,stooke2021decoupling,okada2021dreaming} and intrinsic motivation \citep{guo2021geometric,yarats2021reinforcement,li2021learning,aubret2021distop}.
 
 
\section{Methods}


% \renewcommand{\arraystretch}{1.3}
% \begin{table}[t]
%     \centering
%     \footnotesize
%     %\scriptsize
%     %\tiny
%     {\color{red}\begin{tabular}{lcccc}
%         %\hline
%         \toprule
%         Natural interaction & 3DShapeE & VHE & ToyBox & CORe50 \\ %\hline \hline
%         \midrule
%         Ego-motion & No & Yes &  No &  Yes \\
%         Object manipulations (rotations \& translations) & Yes & Yes & Yes & Uncontrolled  \\
%         \bottomrule
%     \end{tabular}}
%     \caption{\rebut{The different natural interactions studied within each environment and dataset. ``uncontrolled'' refers to the impossibility to isolate the natural interactions from others.}}
%     \label{tab:sumup}
% \end{table}

Our goal is to study the potential of \rebut{time-based augmentations during} natural interactions with objects for \rebut{visual representation learning} and to evaluate the utility of the learned representations for object categorization.\footnote{The source code will be made publicly available.} \rebut{We focus on two kinds of natural interactions: object manipulations (3D translations and rotations) and ego-motion.} %For each of them, we instantiate two complementary training setups.}
\rebut{We introduce two computer-rendered environments, the {\em Virtual Home Environment} (VHE) and the {\em 3D Shape Environment} (3DShapeE) to compare and disentangle the effects of these different types of natural interactions.}

\rebut{We also validate our findings using two real-world first-person video datasets. The ToyBox environment \citep{wang2018toybox} permits studying the relative benefits of object translations and rotations. The CORe50 environment \citep{lomonaco2017core50} allows us to explore the effects of smooth visual tracking and to mimic the effects of ego-motion.}
%In the next sections, we describe our setups in detail\footnote{The corresponding source code will be made publicly available.}.

%with the . In the VHE, an agent moves in a near-photorealistic house while handling the same object. In 






%\rebut{One environment, called {\em Virtual Home Environment} (VHE), enables us to precisely control both object manipulations and the ego-motion} that feed our time-based SSL algorithm. Thus, we can properly disentangle the relative benefits of each kind of natural interaction. In this environment, an agent can ``play'' with thousands of textured objects in a computer-rendered near-photorealistic house. The agent turns its body while continuing to look at the same object, switches the held object without turning its body, turns and varies the distance of the objects. \rebut{To better study the impact of object manipulations on shape generalization only, we introduce a second environment called {\em 3D Shape Environment} (3DShapeE).} It replicates the VHE environment, but incorporates untextured objects and a blank background. 

%Two additional datasets allow us to validate our findings on real-world object footage. First, we test our method on the ToyBox environment \cite{wang2018toybox} to validate our findings on first-person view multifaceted manipulations of objects. Second, we consider the CORe50 dataset of videos of first-person view object manipulations \citep{lomonaco2017core50} and refer to this environment as the {\em CORe50 Environment}. It incorporates realistic object manipulations and  \rebut{ego-motion with} smooth visual tracking of objects. By dynamically reordering the frames of videos, we study how the resulting temporal structure of interactions shapes meaningful object representations in a time-based self-supervised learning framework. In the next sections, we describe our setups in detail\footnote{The corresponding source code will be made publicly available.}.

%\tableautorefname~\ref{tab:sumup} sums up the role of each setup. In the next sections, we describe our setups in detail\footnote{The corresponding source code will be made publicly available.}.


%To dissect the roles of different time-based augmentations and to validate our approach on real-world video data, we instantiate two complementary training setups. We highlight the main role of each dataset in \tableautorefname{tab:sumup}.

% Two environments enable us to precisely control the kind of objects and the kind of interactions that feed our time-based SSL algorithm, and thus to properly disentangle their relative benefits. In the first environment, called {\em Virtual Home Environment} (VHE), an agent can ``play'' with thousands of textured objects in a computer-rendered near-photorealistic house. The agent turns its body while continuing to look at the same object, switches the held object without turning its body, moves its gaze and adapts focus distance (accommodation), turns and varies the distance of the objects. The second environment, called {\em 3D Shape Environment} (3DShapeE), replicates the first one, but incorporates untextured objects and a blank background. It aims to study the impact of natural interactions with objects on shape generalization only.

% The second environment, called {\em 3D Shape Environment} (3DShapeE), replicates the first one, but incorporates untextured objects and a blank background. It aims to study the impact of object manipulations with objects on shape generalization only.

% Two additional datasets allow us to validate our findings on real-world object footage. First, we test our method on the ToyBox environment \cite{wang2018toybox} to validate our findings on first-person view multifaceted manipulations of objects. Second, we consider the CORe50 dataset of videos of first-person view object manipulations \citep{lomonaco2017core50} and refer to this environment as the {\em CORe50 Environment}. It incorporates realistic object manipulations, \rebut{ego-motion and} smooth visual tracking of objects. By dynamically reordering the frames of videos, we study how the resulting temporal structure of interactions shapes meaningful object representations in a time-based self-supervised learning framework. In the next sections, we describe our setups in detail\footnote{The corresponding source code will be made publicly available.}.


\subsection{Virtual Home Environment}\label{sec:virtualhome}

%\paragraph{Object interactions in near photo-realistic houses.}\label{sec:objint}

% \cite{aubret2022embodied} recently proposed to place an embodied agent within an environment that resembles a residential house, where it can \textit{play} with objects and change positions. Figure \ref{fig:house} depicts a bird's eye view showing the floor plan of aforementioned house. The interactions take place on two timescales. First, the agent is spawned in a randomly sampled location and engages in a 100-timesteps-long episode (or session). According to the agent's location, they sample between two and six objects from a predefined set of 20 objects and randomly place them around the agent. Their position in the world determines what background is in the field of view. Each background contains unique static objects and floor/wall textures. Second, at every timestep the agent is presented with the choice of either turning its body towards another object (to the right or left) or keep fixating on the current object. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{iclr_rebuttal_images/new_env5_alt_tight2.jpg}
    \caption{Top view of the VHE used to situate our agent in a house. Blue triangles/orange circles show possible agent/object positions, respectively. In this episode, the agent is located in the office (blue arrow) and interacts with a plush toy. Successive first person views of object interactions are shown in the lower left.}
    \label{fig:house}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{iclr_rebuttal_images/Figure2.pdf}
    \caption{Examples of time-based augmentations while ``playing'' in the VHE (left, A-C): A) object rotation; B) ego-motion; C) depth change. CORe50 (right, D-E): D) close-by frames of objects in 2 different recording sessions; E) different exemplars of the object category ``cellphones'' shown in different contexts. ToyBox (left, F-H): F) depth change, G) lateral translation, H) object rotation.}
    \label{fig:example_trans}
\end{figure}

To simulate \rebut{a diverse set of} natural interactions of an infant in its home, we take inspiration from \citep{aubret2022toddler} and place an agent within an environment that resembles a residential house, where it can ``play'' with objects and change positions. Figure~\ref{fig:house} depicts a bird's eye view showing the floor plan of the aforementioned house. In comparison with \citet{aubret2022toddler}, we integrate a two order of magnitude higher number of fully textured toy objects, as well as novel interactions with these objects.
%The interactions take place on two timescales. First,
The agent is spawned in a randomly sampled location, staying there for 100-timestep-long episodes (or sessions). Its position in the world determines what background will be seen. Each background contains a unique combination of static objects and floor/wall textures. %Second, at every timestep the agent is presented with the choice of either selecting another object or keep interacting with the current object. 

\paragraph{Toys4k dataset.} The \rebut{agent interacts with objects from the} Toys4k dataset, \rebut{which} is composed of 4,179 diverse 3-D toy objects distributed in an unbalanced way into 105 categories \citep{stojanov2021using}. It was designed to match the objects typically encountered by infants. We place textured objects in different locations of the full house. We modify/remove 3D models, only keeping quick-to-process and correct-quality objects in our simulations (cf. \appendixautorefname~\ref{app:3dobjects} for more details). To study the ability of our agent to generalize over categories, we use two thirds of the objects of each category for training and keep the last third for testing. We construct a test set composed of $5$ randomly rotated views of the test objects in different locations of the house. Except for rotation, no additional transformations have been applied to build the test set. We also introduce 3 novel houses to test the robustness of the object-representation with respect to novel out-of-distribution backgrounds (cf. \appendixautorefname~\ref{app:newhouses}).
%we generate $3$ randomly rotated views of the test objects when the agent does not move (3D Shape Environment) and $5$ when it moves in a house environment (see section on ego-motion below)
% We verify in \appendixautorefname~\ref{app:onerot} that this does not bias our evaluation.




%To assess the impact of our augmentations, we setup another a \textbf{3D Shape Environment} in addition to the full house environment. In the first one, the agent interacts with grey objects in front of a fully white background. This marginalizes the possible impact of background and colors. %Second, we let the agent interact with colored objects without moving. This aims to isolate the impact of interactions on the background.


%\paragraph{Overview of the natural interactions}
%
%Using the houses and the toys, we analyze the impact of three ways to influence time-based augmentations:
%We want to simulate infant-like interactions, these include:
%2) slow/quick object manipulations; 1) ego-motion with slow/quick background changes while holding the same object.  We describe each of them below.
%These might contribute differently to the representation learnt through time-based SSL. We describe each of them below. %We also discuss gaze control in \appref{app:gaze}. 

%(cf. \appref{app:gaze})

%(BARELY ANYTHING TO BE SEEN HERE) in C -> if you still would like to change that
%Unlike \citet{aubret2022embodied}, we do not sample all objects of the location at the beginning of the episode.

\paragraph{Object manipulations.} At only a few months old, infants start to hold objects and \rebut{move and }rotate them \citep{byrge2014developmental}. \rebut{Similarly, our} agent can manipulate the objects in two different ways. First, it can rotate the object around the vertical axis (yaw) \rebut{by a random} angle \rebut{drawn uniformly from the interval} $[0, \text{rot}]$ degrees, \rebut{where the} hyperparameter $\text{rot}$ \rebut{sets the} maximal \rebut{speed of object rotations} (cf. \figref{fig:example_trans}A). Second, the agent can also bring the object closer or move it further away, as shown in \figref{fig:example_trans}C; we model this as a change of distance uniformly sampled from $[-d, d]$, \rebut{where $d=\SI{7.5}{cm}$ is the maximal distance change.} The distance is bounded between $\SI{0.65}{m}$ and $\SI{1.1}{m}$ to reflect morphological limitations of the agent's arms.

\paragraph{Ego-motion.} When infants \rebut{become mobile}, they can play with objects while moving in their environment. To simulate this, our agent can turn its body towards a neighboring location while \rebut{holding} the same object \rebut{so that it is seen against a different background}.
%By avoiding displacement across possible agent locations, we keep the backgrounds temporally consistent, as typically experienced by humans.
As shown in \figref{fig:example_trans}B, \rebut{the new} background \rebut{will usually have} similar floors and walls. \rebut{Sometimes an infant will also engage with a new object.} We model \rebut{both possibilities} by deterministically turning \rebut{the agent} every $N_{\rm s}$ timesteps and switching \rebut{to a new} object with probability $1-p_{\textrm{o}}=0.1$. A small/medium $N_{\rm s}$ respectively simulates in an unnatural/natural fashion an agent that always/sometimes moves with its object. When this egomotion is disabled, the agent simultaneously picks up a new object and turns every $N_{\rm s}=10$ timesteps. For some experiments (\tableautorefname~\ref{tab:main_results} and \figref{fig:persession_ablation}A, B), we also allow the agent to visit another room every $N_{\rm s}$ steps while continuing to interact with the same object. \rebut{This allows us to investigate the effect of more drastic background changes, but may be a less valid model of a human infant's interaction with objects.}


%First, as shown in \figref{fig:example_trans}C, it may lower or lift the object by an amount drawn uniformly from $[-0.1 , 0.1]$ meters, with lower/upper bounds at $0$ and $0.5$ meters.


% \paragraph{Gaze control} In humans, gaze control through saccades occurs on a faster timescale than object control/ego-motion. Therefore, we assume the agent can instantaneously reset the gaze position while it only progressively changes the object in front of it and its own position.

% First, to simulate saccadic eye movements \citep{trukenbrod2019spatial}, we enable the rotation of the camera towards a given angle around the object position. The apparent effect is a motion of both the background and the object (see \figref{fig:example_trans}A). The agent uniformly samples pan and tilt angles in $[-A;A]$, where $A$ is a hyper-parameter that defines the maximal saccade angle. Second, humans have a limited depth of field and need to adapt the shape of their lens to the distance of the fixation point, also called focus distance. As a consequence, the fixation point appears sharp in the visual field, while stimuli before and behind the fixation point are increasingly blurred. We model this by allowing the focus distance to range in $[0.47;1.87]$ meters. We display the effect in \figref{fig:example_trans}B. At object initialization or when this feature is disabled, we apply the perfect strategy of always focusing on the object.

% \paragraph{Intuition.} Why should it work ? 
% To assess the quality of our representation, we train a linear  on top of the representation in a supervised fashion \citep{chen2020simple}. Because of the limited buffer size, the training data changes over time. To prevent the impact of such shift on the evaluation, we train the linear probe on the test set. While the result could be different from a classifier learned on the training data, preliminary experiments showereadoutd similar evaluation results in this environment. It also makes possible to evaluate the linear separability of unseen objects in \figref{fig:flipvsrot}B. We average all results over 3 random seeds. Hyper-parameters are given in the \appref{app:hyperparameter}.
 
\subsection{3D Shape Environment}

In order to study the influence of natural interactions on shape generalization while \rebut{minimizing} the impact of object colors or background, we introduce a simple 3D Shape Environment (3DShapeE). \rebut{It differs from the VHE in two respects}: 1) we import untextured versions of toy objects from the Toys4k dataset, making them appear grey;  2) we place the agent in an empty environment so that objects are seen against a blank background. \rebut{Examples of inputs are given in \figref{fig:flipvsrot}E and augmentations are the same as in the VHE environment (\figref{fig:example_trans}A-C).}


\subsection{ToyBox Environment}\label{sec:toyboxdataset}

The ToyBox dataset \citep{wang2018toybox} contains first-person videos of an observer manipulating 360 objects (12 categories, 30 objects each). In each clip, a person applies one type of transformation: a translation (x, y or z), rotation (around x, y or z axis), a ``hodgepodge,'' nothing specific, or in some cases, nothing if there is no object. We sample two frames per second from each clip (cf. \appref{app:toyboxdataset} for more details).
%Unlike in the CORe50 environment (see below), we only focus on the impact of object manipulations on time-based augmentations.
\rebut{Two successively sampled frames form} a positive pair. At the end of a clip, a positive \rebut{pair if formed from the last frame sampled from the clip and} the first image of the randomly sampled next clip. 

\subsection{CORe50 Environment}

The CORe50 dataset \citep{lomonaco2017core50} contains first-person views of an observer manipulating objects. The dataset comprises 167,866 images of 50 different objects belonging to 10 distinct object categories. All objects were filmed in 11 sessions corresponding to different natural environments. The images from all but one object per class \rebut{are used to form} the training \rebut{and validation} sets. \rebut{Specifically, every 10th image enters the validation set, the others form the training set}. The images of the \rebut{held-out} object \rebut{of each} class \rebut{form the test set}. This \rebut{allows us to test} generalization \rebut{to unknown} objects \rebut{from familiar} categories.
%but also investigate how much of the background and object-specific information is encoded in the learnt representation.

%Using this dataset, we approximate different kinds of natural interactions: 1) the number of fixations on an object; 2) ego-motion with slow/quick background changes while holding the same object; 3) The speed of object manipulation. We describe each of them below.

\rebut{The videos in this dataset show real object manipulations, but we also use it to mimic the effects of ego-motion through the way we sample images from the different video clips. In general, successively sampled images form positive pairs. We create sequences of images by starting from a particular frame of one of the video clips showing an object manipulation and defining a probability $p_{\textrm{o}}$ that the manipulation of the same object continues. Otherwise an interaction with a new object will start. In case the interaction continues, the next frame in our sampled sequence will be randomly chosen as either the next or the previous frame in the video clip. Thus, as long as the object manipulation continues, the sampled sequence of frames corresponds to a random walk through the frames of the video. A high/low $p_{\textrm{o}}$ leads to long/short random walks. Specifically, the expected number of successive frames $N_o$ showing the same object is given by:}
\begin{equation}
    \mathbb{E}\left[ N_{\textrm{o}}|p_{\textrm{o}} \right] = 1 + \sum_{x=0}^{\infty} x p_{\textrm{o}} ^x(1- p_{\textrm{o}}) = 1 + \frac{p_{\textrm{o}}}{1-p_{\textrm{o}}} \; .
\end{equation}

%Using this dataset, we approximate different kinds of natural interactions: 1) ego-motion with \rebut{rare/frequent} background changes while holding the same object; 2) The speed of object manipulation. \rebut{We also analyse the impact of object manipulation duration on the representation, \textit{i.e.} the number of consecutive frames spent manipulating the same object.} We describe each of them below.

%\paragraph{Object manipulation duration.}
%Here we simulate the different amount of time an infant plays with an object. For every sampled image, the probability that the positive pair is from the same object is given by $p_{\textrm{o}}$. It means we model the duration of object manipulation $N_{\textrm{o}}$ as a sequence of independent Bernoulli trials given a predefined probability, which yields

%as the expected value of \rebut{object manipulation duration} before taking another object. %$N_{\textrm{o}}$ plays an analogous role to choosing the frequency of object-oriented manipulations in the VHE.

%\paragraph{Ego-motion.} We propose to simulate an infant that moves with objects in its environment while holding the same object. Thus, similarly as above,
\rebut{To mimic the effects of ego-motion causing an object to be seen against changing backgrounds, we also define a probability $p_{\textrm{s}}$ that the sequence of views stays within the same session, i.e., the same video clip.} Thus, there is a chance of $1 - p_{\textrm{s}}$ that the sequence of views of the same object ``jumps'' to a different video clip showing the same object in a different context. In this case, a positive pair is generated from two images of the same object recorded in different recording sessions. This cross session sampling (CSS)
%simulates the behaviour of taking an object to another room and naturally takes place on a slower timescale than \rebut{object manipulation duration}. $N_{\textrm{s}}$
is analogous to the role of ego-motion in the VHE.

\rebut{As an alternative to the random walk procedure described above we also consider a variant where the next view of the same object is chosen uniformly at random from the current video clip. This leads to images forming a positive pair, which stem from distant time points in the original video clip. While this is not a realistic model of viewing sequences experienced by an infant, it allows us to assess the benefits of positive pairs containing more distinct views of the same object. This is analogous to greater speed of object rotation in the VHE.}

%\paragraph{Speed of object manipulation.}
%To simulate the different speed of object manipulations in humans, we distinguish two different ways of how the next view (or positive image) of the {\em same} object is sampled during \rebut{object manipulation}. Our default method is called {\em random walk} view sampling. Here, the next view of an object is chosen to be one of the two adjacent video frames. The second method is the {\em uniform} view sampling. Here, the next view is picked uniformly at random from the same session. It approximates a higher manipulation speed, but without impacting either the marginal probability distribution of each sample or the expected \rebut{object manipulation duration}. This approach provides the most diversity among successive views, which is expected to aid learning, but is less congruent with an infant's viewing experience.
%not meant to simulate an infant's viewing experience.

%\paragraph{Sampling procedure.} 

%Note that inter-object switches \rebut{occur in time-based augmentations during natural interactions}.
For implementation details \rebut{of our sampling procedure} see \appref{app:core50app}. In \rebut{brief, it is an extension of the procedure used in} \citet{schneider2021contrastive} \rebut{to allow CSS.}
%order to technically apply our method while controlling the parameters $N_o$ and $N_s$, we use a procedure similar to  and extend it to account for background changes.

%We generate positive pairs with $N_o$ and $N_s$$ These pairs fill a buffer which then serves to randomly generate batches of data.  Note that the re-sampling is not part of the learning, but a tool to generate video with specific temporal statistics and to study how time-based augmentations cope.

%In the ``One augmentation'' experiment of \figref{fig:bigexp}, we pre-generate the SimCLR composition of augmentations of each image and do not retransform the images during training, similarly to the VHE.




% Specifically, for each image $i_t$, we sample its time-based positive $i_{t+1}$. When $t+1$ exceeds the time limit of the clip, we sample the first image of a randomly sampled other clip.

%Specifically, for each image $i_t$, we sample its time-based positive $i_{t+\Delta T}$ where $\Delta T \in [1, $K$] with $K$ an hyper-parameter denoting the maximal speed. Let us note $i_{\text{max}}$ the last image of the clip of $i_t$, if $i_{t+\Delta T} > i_{\text{max}}$ there are two cases: if $i_{\text{max}} = i_t$, the next pair is randomply sampled among the first image of all clips; otherwise we set $i_{\text{max}}$ to be the positive pair.

\subsection{Evaluation and training procedure \rebut{for all environments}}\label{sec:evalprocedure}

\paragraph{Learning algorithms.} We consider three SOTA representatives of existing \rebut{algorithms for} data-augmented SSL: SimCLR for contrastive learning \citep{chen2020simple}, BYOL \citep{grill2020bootstrap} for distillation-based methods and VICReg \citep{bardes2022vicreg} for entropy maximization methods. \rebut{We refer to the versions of these algorithms using time-based augmentations as, e.g., SimCLR through time (\textbf{SimCLR-TT}), etc.\ \citep{schneider2021contrastive}.}

\paragraph{\rebut{Positive pair construction.}} \rebut{We consider three ways to augment an image. First, we consider time-based augmentations during natural interactions (\textbf{SimCLR-TT}, etc.). For this, unless stated otherwise, we set the positive pair of a source image as the next image in the temporal sequence. Second, as a comparison baseline, we augment a sampled image with a widely adopted SOTA set of augmentations \citep{chen2020simple,shijie2017research}, \textit{i.e.} crop/resize, grayscale, color jittering and horizontal flip with their default parameters, except for the crop/resize augmentation (cf. \appref{app:hyperparameter}). Third, we propose to combine the two kinds of augmentations (\textbf{SimCLR-TT+}, etc.). For this we apply the conventional SOTA augmentations to the image that temporally follows the sampled source image.} \rebut{We refer to \figref{fig:stimulis} for examples of the different ways to augment source images.} 

% \subsection{Training data in the VHE}\label{app:stimulis}

% \rebut{\figref{fig:stimulis} shows examples of sequential inputs according to the rotation speeds (Inputs) and the results of augmentations according to the augmentation method.}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{iclr_rebuttal_images/stimulis5.pdf}
    \caption{\rebut{Sequences of input images during object rotations (\text{rot}(360)) and egomotion and their augmented positive pair according to the augmentation method (same column). \textbf{Baseline} refers to conventional augmentations; \textbf{*-TT} refers to time-based augmentations; \textbf{*-TT+} refers to combined augmentations.}}
    \label{fig:stimulis}
\end{figure}
% To compare time-based augmentations during natural interactions to conventional image transformations, we augment a sampled image with a widely adopted SOTA set of augmentations \citep{chen2020simple,shijie2017research}, \textit{i.e} crop/resize, grayscale, color jittering and horizontal flip with their default parameters, except for the crop/resize augmentation (cf. \appref{app:hyperparameter}). 

%In the ToyBox environment, VHE and 3DShapeE, the number of time-based augmentations is smaller than the possible number of conventional augmentations. 
\paragraph{\rebut{Controlling for the number of augmentations.}} While we can generate an arbitrary number of positive pairs from one sample image with conventional augmentations, we only have access to one positive time-based pair per sample image for the VHE, 3DShapE, and the ToyBox environment. \rebut{To control for the impact of the number of positive pairs, we \rebut{therefore} only construct one positive pair per sample for all algorithms and augmentation methods:} 1) for the ToyBox environment, we sample positive pairs from a pre-built dataset of the same size as the original one, but composed of conventionally augmented images; 2) for the VHE and 3DShapeE the agent collects images, augments them and stores them in a buffer of size $100{,}000$. It simultaneously trains on images randomly sampled from the buffer at every timestep. We show in \appref{app:augnumber} that controlling for the number of augmentations does not impact the results of our analysis.

\paragraph{\rebut{Controlling for the number/distribution of source images.}} \rebut{We want to make sure that we compare the quality of the augmentations, and not the amount/diversity of data that feeds the SSL algorithms. Thus, for the comparison baseline, we consider the same natural interactions to generate source images, but we do not use temporal information to generate the positive pairs. This ensures that the number/distribution of non-augmented images is exactly the same across methods (source images in \figref{fig:stimulis}). We make an exception with depth changes in 3DShapeE since we found it to be harmful for the baselines.}

%apply the conventional data-augmentations on the same temporal sequence as for time-based augmentations during natural interactions
%Thus, we also rotate the object for conventional augmentations (but do not consider it as an augmentation). When we study the combined effect of the two types of augmentations, we apply the sequence of conventional augmentations to the next image in the temporal sequence. We show in \appref{app:augnumber} that limiting the number of conventional augmentations does not impact our analysis. %We study the impact of this restricted number of conventional augmentations in \appref{app:augnumber}.
%To make a fair comparison, we need to 
%In the ToyBox environment, VHE and 3DShapeE, the number of time-based augmentations is smaller than the possible number of conventional augmentations since we do not generate a new time-based augmentation for each training batch. In addition, we want to make sure we compare the quality of the augmentations, and not the amount/diversity of data and augmentations that feeds the SSL algorithm. 



% thus we limit the number of conventional data-augmentations :
\paragraph{Evaluation.} \rebut{We compute the representation with a ResNet18 on ToyBox and CORe50 and with a simpler convolutional neural network on 3DShapeE and VHE.} We evaluate the learnt representation after 480,000 steps for the VHE and 3DShapeE, 60 epochs for ToyBox and 100 epochs for CORe50. The quality of the learned representation is assessed by training a linear readouts on top of the learned representation in a supervised fashion \citep{chen2020simple}. \rebut{Depending on the question, we train linear readouts to either predict the identity of an object, the category of an object, or the location/session of the object.} We average all results over 3 random seeds. Because of the small number of objects per category in the CORe50 dataset, we apply a cross-validation with 5 splits. Hyperparameters are given in \appref{app:hyperparameter}.


 %We use a relatively high depth of field (distance range where objects produce a sharp image) to make sure SimCLR does not access less low-frequency information about the object than SimCLR-TT.

%While \citet{chen2020simple} randomly and independently applies each data-augmentation with a fixed probability, unless stated otherwise, we always apply our time-based augmentations ($p=1$).

\section{Results}\label{sec:results}

In this section, we \rebut{first} study the benefits of using time-based augmentations \rebut{during} natural interactions \rebut{with objects for} self-supervised \rebut{visual representation }learning.
%we compare the impact of conventional data augmentations to augmentations derived from natural interactions in the context of self-supervised methods. 
Then, we provide an in-depth analysis of the impact of \rebut{3-D} object rotations and ego-motion on the learned representations. An ablation study is \rebut{performed} in \appref{app:com_analysis}.

\subsection{Time-based augmentations derived from natural interactions boost performance of SSL}
\label{ssec:time-based}
%\laentation of objects, and tested on the same orientation of test objects. B.
%Test category accuracy with a linear classifier trained on the multi-view dataset (several orientations
%of objects), and tested obel{sec:comparison}

In \tableautorefname~\ref{tab:main_results}, we compare the quality of the learnt representation when using conventional data-augmentations (SimCLR, BYOL, VICReg), time-based augmentations (*-TT), and their combination (*-TT+) in our \rebut{four test} environments. \rebut{We observe that \rebut{our combined approach (*-TT+)} increases the average test category accuracy with respect the the baselines (SimCLR, BYOL, VICReg) by a range of $[0.037; 0.266]$ points across all environments and all SSL methods. To formally validate our approach, we ran additional runs for SimCLR and SimCLR-TT+ and subsequently applied a t-test on the hypothesis ``SimCLR-TT+ is superior to SimCLR''. We find $p < 0.05$ in our four test environments, thereby confirming our analysis.} Time-based augmentations during natural interactions \rebut{(*-TT)} do not perform very well on their own, presumably because they \rebut{do not create invariance to color/grayscale changes in our test environments} (cf. \appref{app:com_analysis} for ablation studies of augmentations). In the next sections, we analyse the impact of 3-D rotations and egomotion on the learnt representations.

%Time-based augmentations outperform standard data-augmentations on the 3DShapeE (except for VICReg which shows a high variance) and the VHE, but not consistently in other environments. This suggests that while they are mostly crucial for shape generalization, they may be over-sensitive to object colors, like the crop/resize data-augmentation \citep{chen2020simple}.
%In VHE, while SimCLR-TT may also be sensitive to object colors, we presume that SimCLR is even more sensitive to background details. We further study shape generalization in \secref{sec:rotations} and the encoding of the background in \secref{sec:motion}. Importantly, we observe that the combination of augmentations consistently outperforms conventional data-augmentations. In the next sections, we analyze the impact of rotations and speed of motion on the learnt representations.

\renewcommand{\arraystretch}{1.3}
\begin{table}[t]
    \centering
    \footnotesize
    %\scriptsize
    %\tiny
    \begin{tabular}{lcccc}
        %\hline
        \toprule
        Method & VHE & 3DShapeE & ToyBox & CORe50 \\ %\hline \hline
        \midrule
        SimCLR & $0.328 \pm 0.002$ & $0.527 \pm 0.005$  &  $0.313 \pm  0.001$ & $0.544 \pm 0.074$ \\
        SimCLR-TT  & $0.369 \pm 0.005$  & $0.598 \pm 0.007$& $0.189 \pm 0.009$ & $0.449 \pm 0.152$ \\ %\hline
        SimCLR-TT+ & $\mathbf{0.537 \pm 0.001}$ & $\mathbf{0.621\pm 0.001}$  & $\mathbf{0.378 \pm 0.005}$ & $\mathbf{0.610 \pm 0.090}$\\ 
        \midrule
        BYOL  & $0.352 \pm 0.017$ & $0.496 \pm 0.012$ & $0.354 \pm 0.007$ & $0.552 \pm 0.063$   \\ %\hline
        BYOL-TT &  $ 0.369 \pm 0.007$ &$\mathbf{0.570 \pm 0.001}$ & $0.213 \pm 0.014$ & $0.448 \pm 0.160$\\ %\hline
        BYOL-TT+ & $\mathbf{0.516 \pm 0.002}$ & $0.536 \pm 0.001$  & $\mathbf{0.393 \pm 0.031}$ & $\mathbf{0.614 \pm 0.128}$\\ %\hline\hline   
        \midrule
        VICReg & $0.169 \pm 0.006$ & $0.512 \pm 0.002$ & $0.381 \pm 0.019$&$0.410 \pm 0.073$ \\ %\hline
        VICReg-TT & $0.264 \pm 0.012$ & $0.383 \pm 0.167 $   & $0.158 \pm 0.008$ & $0.245 \pm 0.084$\\ %\hline
        VICReg-TT+ & $\mathbf{0.435 \pm 0.013}$ & $\mathbf{0.574 \pm 0.008}$  & $\mathbf{0.418 \pm 0.016}$& $\mathbf{0.503 \pm 0.057}$\\ %\hline \hline
        \bottomrule
        %\multicolumn{5}{l}{\scriptsize{$^\dagger$ based on 3 training/testing splits}}%,  $^\ddagger$ based on 2 training/testing splits}}\\
    \end{tabular}
    \caption{Top 1 accuracy $\pm$ standard deviation (over 3 seeds, CORe50 over 5 training/testing splits) under linear evaluation of previous SOTA (BYOL, SimCLR, VICReg) versus our time-based augmentations (*-TT) and their combination (*-TT+). In 3DShapeE, \textbf{*-TT+} use crop/resize, color jittering and rotations. In VHE, \textbf{*-TT+} use rotations, Ns=1 with room changes, color jittering and gray scaling. In both VHE and 3D Shape Environments, \textbf{*-TT} use rotations, Ns=1 with room changes (VHE only) and depth changes. In CORe50 we use $p_s = 0.5, p_o= 0.9$. We refer to \appref{app:abla_syne} for the ablation study that motivates these choices. In ToyBox, we always apply all their respective transformations. Unlike \textbf{*-TT+}, we apply all standard augmentations for the baseline, as we found that removing some of them (crop/resize and flip) was harmful.% (\textit{e.g.} $0.4930971 \pm 0.010842151$ for 3DShapeE).
    }
    \label{tab:main_results}
\end{table}


% \begin{figure}
%     \centering

%     \includegraphics[width=0.51\linewidth]{images/toybox_res.pdf}
%     \includegraphics[width=0.48\linewidth]{images/Figure4_2_widthcompressed.pdf}
%     \caption{A. Comparison between natural augmentations (Time), conventional augmentations (SimCLR aug) and the combination of both for the VHE. Time-based augmentations are labeled by the changes they induce: D=depth,  Ro=room changes. Shaded areas represent one standard deviation (over different random seeds). B. Test category accuracy on ToyBox. T=Time; J=Color Jittering; G=Grayscale; B=Blur; H=Horizontal flip; C=Crop/Resize. \textit{One aug} refers to one augmentation per sample (cf. \secref{sec:toyboxdataset}).} C and D: Category accuracy for the CORe50 Environment, $p_{\textrm{s}}=0.95$. C. Validation set accuracy compared to the baselines supervised (grey) and SimCLR (purple). D. Same for test set. Shaded areas represent one standard deviation of test category accuracy over 3 seeds.

%     \label{fig:bigexp}
% \end{figure}
    %Shaded areas in B and C correspond to one standard error based on 3 random seeds or 2 fold cross-validation with different train/test splits, respectively.}
    %\includegraphics[width=0.29\linewidth]{images/best_v2p.pdf}
    %\includegraphics[width=0.70\linewidth]{images/Figure4_2_final.pdf}
%\begin{figure}
%    \centering
%    \includegraphics[width=0.5\linewidth]{images/example_res.pdf}
%    \caption{Test category accuracy according to the used augmentations after 50 training epochs. We note T=Time, J=Color Jittering; G=Grayscale; B=Blur; H=Horizontal flip; C=Crop/Resize. \textit{One aug} refers to the use of one composition of augmentation per sample (cf. \secref{sec:toyboxdataset})}
%    \label{fig:my_label}
%\end{figure}

% just for demonstration purposes 1x4
%\begin{figure}
%    \centering
%    \includegraphics[width=0.49\linewidth]{images/Figure4_2_widthcompressed.pdf}
%    \includegraphics[width=0.49\linewidth]{images/Figure4_2_widthcompressed.pdf}
%    \caption{}
%    \label{fig:nolabel}
%\end{figure}

% \textbf{Right:} Ablation analysis of all data-augmentations according to whether objects are textured, colored and in front of several backgrounds. The combinatorial combination of all augmentations being computationally infeasible, we progressively accumulate augmentations. Horizontal bars indicate the minimum and maximum average accuracy over seeds. 

% A large-scale study of the combinatorial effect of all these augmentations is beyond the scope of the paper, thereby we focus our comparison with the widely used set of augmentations \cite{chen2020simple,shijie2017research}.

\subsection{Object manipulations including 3-D rotations support shape generalization}\label{sec:rotations}
%Show Simclr + rotation + ablation with flip.
% show the tempral curve for flip ablation
% show simclr + rotations for all backgrounds MISSING

%Core 50, ablation on random vs uniform sampling
%TDW ablation on speed rotation
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{images/core50_sampling_ablation.pdf}
%     \caption{Class accuracy for the CORe50 dataset, $p_{\rm persess}=0.95$. A) Validation set accuracy compared to the baselines supervised (grey) and SimCLR (purple). B) Same for test set. Shaded area corresponds to standard error based on 3 fold cross-validation with different train/test splits.
%     }
%     \label{fig:exp43}
% \end{figure}

 %\figref{fig:flipvsrot}A show that removing augmentations based on translations (-Ho,Tr) and rotations (-Ho,R) both hurt the quality of the representation. Interestingly, removing some of them only (-Ho) do not affect the performance, presumably because other interactions a. %the information about the shape is still provided by other interactions.
%made an ablation study in the ToyBox environment and

%VHE. We let the agent interact with untextured (grey) versions of the objects, which are seen against a white background.  %Figure \ref{fig:core50augfix}B depicts the influence of the number of fixations regarding the different training scheemes. 
To assess the importance of object manipulations to generalize over object shapes, we conducted experiments in 3DShapeE. \figref{fig:flipvsrot}A shows that increasing the speed of object rotations systematically increases the category recognition accuracy. Similarly, in the CORe50 Environment (\figref{fig:flipvsrot}D) the uniform sampling of views clearly outperforms \rebut{the default} random walk \rebut{sampling procedure}, in particular for short \rebut{object manipulations (low $p_o$)}. Interestingly, we observe the inverse effect on individual object recognition accuracy (\figref{fig:flipvsrot}B). We conclude that fast object rotations (in the extreme case constructing positive pairs from randomly rotated views of an object) tend to discard object-specific details and focus the representation on \rebut{more general shape features}, which will be similar for different objects of the same category. 

%Next, we \rebut{investigate} how object rotations relate to the standard horizontal flip augmentation, since the flip resembles a 180-degrees rotation for symmetric objects and uniform background. In \figref{fig:flipvsrot}C, we combine the flip augmentation and object rotations with other conventional augmentations. We see that when the object rotation speed is large enough ($rot(360)$), there is no additional benefit in using the horizontal flip augmentation. However, rotations always boost performance compared to the pure flipping augmentation. Thus, we conclude that using 3-D object rotations rather than flipping results in considerably better representation of object shape. % it shows that 1- horizontal fliping is important because it simulates object rotations; 2- using rotations rather than flipping results in considerably better shape-oriented representations.

Finally, we \rebut{investigate} the relation between rotation invariance and object shape. To do so, we design a new test setup. In the \textit{single-single setup}, we train the linear classifier on the representations of a single-view dataset that contains \rebut{only} one view from a common orientation for each training object (back, side, \dots). We assess \rebut{the classifier} on \rebut{images of} the test objects shown in same orientation. This means that the linear classifier can not learn the invariance to rotation and does not \textit{explicitly} need it for classification. We consider datasets of orientations of -90° (front view), -45° (\nicefrac{3}{4} view), 0° (side view) as they contain the extreme cases in terms of the amount of visible surface \citep{blanz1999object}. %our preliminary results. %We do not show other datasets for the sake of visualization.% Second, in the \textit{multi-single setup}, we train a linear classifier on representations gained from the usual multi-view dataset but test it on the single-view datasets.
%First, we observe an overall decrease of performance in SimCLR when testing with the \textit{single-single setup} (\figref{fig:rotbackanalysis}A) in comparison to \textit{multi-single setup} (\figref{fig:rotbackanalysis}B). In contrast, SimCLR-TT+ (with rotations only) is more robust to the training set of the linear classifier. This suggests that the performance of SimCLR is over-estimated due to the linear classifier. 

%However, we also see in \figref{fig:rotbackanalysis}A that the performance of SimCLR-TT+ varies across view-types. We conclude that SimCLR-TT+, despite learning invariance to rotations, does not systematically exploit the most informative view about the category of an object to categorize its different views.

We
%rather
hypothesize that including 3-D rotations in time-based augmentations allows the model to encode \rebut{3-D} shape \rebut{features} in the learned representation, which results in an improved category recognition. To \rebut{test} this hypothesis, we first evaluate category recognition based on several views of an object (thus its whole shape).  In \figref{fig:flipvsrot}C, we compute a majority vote among classification results from the different single-single classifiers as follows: if more views (e.g., 90°, 80°, 10°) are \rebut{classified} as category A than category B (e.g., 0°, -90°), category A is selected. We observe a large increase of accuracy \rebut{for} SimCLR. We conclude that encoding the \rebut{3-D} shape \rebut{improves} category recognition. \rebut{Importantly}, we do not observe such an increase of accuracy for SimCLR-TT+ with the majority vote. We deduce that \rebut{SimCLR-TT+} better \rebut{infers the 3-D} shape of the object from one view, which \rebut{strongly} improves category recognition.  

% We observe a large increase of accuracy in comparison with other views for SimCLR, reaching SimCLR-TT+ performances. 


%In contrast, SimCLR-TT+ only slightly benefits from the majority vote. It exhibits that the proportion of views that agree with the majority vote for SimCLR-TT+ is higher than for SimCLR. Assuming that classifying with the majority vote amounts to categorize according to the 3D shape similarity (equivalently to the similarity over different views), it suggests that SimCLR-TT+ better extrapolates the shape of the object from one view. This turns out to crucially improve category recognition.

% We deduce that 

% a majority vote among different orientations: different objects with a large number of visually similar views become similarly represented. This amounts to compare the shape of objects, which turns out to improve category recognition.

%, presumably because it is hard deduce the shape of an object from particular views (cf \figref{fig:rotbackanalysis}D, back orientation of hats)
% unlike SimCLR-TT+, SimCLR performance depends on the ability of the linear classifier to learn invariance to rotations.
% In \figref{fig:flipvsrot}D, we assess the ability of SimCLR and SimCLR-TT+ (with only rotations as time-based augmentations) to generalize categories on a single orientation of an object.


% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{iclr_images/rotflip.pdf}
%     \includegraphics[width=0.49\linewidth]{iclr_images/rotation_analysis.pdf}
%     \includegraphics[width=0.49\linewidth]{iclr_images/egomotion.pdf}
%     \caption{A. 3DShapeE test category recognition accuracy according to the maximal rotation speed $S$, without other augmentations. B. 3DShapeE test object recognition accuracy according to the maximal rotation speed, without other augmentations. C. 3DShapeE test category accuracy according to different combinations of flip and rotation speeds. The shaded area displays the +/- standard deviation of test category accuracy over seeds. D and E. Impact of the frequency ($N_{\rm s})$ of body motions and whether they change rooms on the final test category accuracy (D) and the final background accuracy (E). We also used object rotations, color jittering and grayscaling. Vertical bars indicate one standard deviation.}
%     \label{fig:flipvsrot}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.74\linewidth]{iclr_rebuttal_images/shapeanalysis.pdf}
    \includegraphics[width=0.24\linewidth]{iclr_images/CORe50_rw_vs_uni.pdf}
    \includegraphics[width=0.98\linewidth]{iclr_rebuttal_images/greyobjects3D2.png}
    \caption{A. 3DShapeE test category recognition accuracy \rebut{for different} maximal rotation speeds $S$, without other augmentations. B. 3DShapeE test object recognition accuracy \rebut{for different maximum} rotation speeds, without other augmentations. The shaded area displays the +/- standard deviation of test category accuracy over seeds. C. Test category accuracy with a linear classifier trained on one single orientation of objects, and tested on the same orientation of test objects. We used 5 seeds, all our conventional augmentations but only rotations ($[0,360]$ degrees) as time-based augmentation. We \rebut{also} apply the majority vote on datasets of six different orientations: 0°, 10°, -45°, 80°, -80°, -90°.  D. Category accuracy for the CORe50 Environment when varying the duration of object manipulations ($p_{\textrm{s}}=0.95$). The shaded area shows $\pm$ standard error. A-D. We used SimCLR-TT. E. Example of three views for eight objects \rebut{from} four categories in 3DShapeE. In order from left to right for each object, we \rebut{show} orientations of: 0° (side view); -45° (\nicefrac{3}{4} view); 90° (back view). The red rectangles \rebut{highlight} visually similar views \rebut{of different objects}.}
    \label{fig:flipvsrot}
\end{figure}

%C. 3DShapeE test category accuracy \rebut{for} different combinations of flip and rotation speeds. 
% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=0.49\linewidth]{iclr_images/rotation_analysis.pdf}
%     % \includegraphics[width=0.49\linewidth]{iclr_images/egomotion.pdf}
%     \includegraphics[width=1\linewidth]{iclr_rebuttal_images/maniptime_egomotion.pdf}
%     \caption{A. Impact of the manipulation duration $N_{\rm o}$ on the final test category accuracy. B and C. Impact of the frequency ($N_{\rm s})$ of body motions and whether they change rooms on the final test category accuracy (B) and the final background accuracy (C). We also used object rotations ($[0,360]$ degrees), color jittering and gray scaling. Vertical bars indicate one standard deviation.}
%     \label{fig:rotbackanalysis}
% \end{figure}

%Show crop ablation
% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{images/test_houses_v2p.pdf}
%     \caption{ Impact of the frequency ($N_{\rm s})$ of body motions and whether they change rooms on the final test category accuracy (A) and the final background accuracy (B) after 420,000 timesteps. Vertical bars indicate one standard deviation.}
%     \label{fig:backgroundanalysis}
% \end{figure}

\begin{figure}
    \centering
    %\includegraphics[width=1.0\linewidth]{images/fig8_3_tight.pdf}
    \includegraphics[width=0.5\linewidth]{iclr_rebuttal_images/backgrounds.pdf}%
    \includegraphics[width=0.5\linewidth]{iclr_rebuttal_images/fig8_3_tight6.pdf}
    \caption{A and B. Impact of the frequency ($N_{\rm s})$ of body motions and whether they change rooms on the final test category accuracy (B) and the final background accuracy (C). We also used object rotations ($[0,360]$ degrees), color jittering and gray scaling. Vertical bars indicate one standard deviation. C and D. Mean CORe50 classification accuracy (SimCLR-TT) dependent on the duration of object manipulations and the frequency of session switches based on 3 training/testing splits.}
    \label{fig:persession_ablation}
\end{figure}

\subsection{Moving with objects mitigates the effect of background clutter}\label{sec:motion}
%Core50 ablation + TDW ablation

To evaluate the impact of ego-motion while holding objects, we trained our agent in the VHE with different levels of motion. In \figref{fig:persession_ablation}A, we see that increasing the frequency $\nicefrac{1}{N_{\rm s}}$ and the range (room) of motion considerably boosts the test category accuracy in backgrounds from training and novel houses. At the same time, we observe a decrease of the accuracy when classifying the background (\figref{fig:persession_ablation}B). We conclude that moving while holding objects improves the representation's invariance with respect to the background. %However, we observe that these two effects are less pronounced for novel backgrounds (blue) from three unfamiliar houses. %In contrast, we see in \figref{fig:bigexp}A that the quantity of motion does not significantly impact the SimCLR performance (compare black and purple curves).

%We hypothesize that adding the color transformations of SimCLR increase the range of backgrounds that do not impact the representation.%Adding SimCLR augmentations reduce the gap between different house performances (\figref{fig:backgroundanalysis} (left)), while slightly limiting the loss of background-related information (\figref{fig:backgroundanalysis} (right)). Thus, we hypothesize that adding the color transformations of SimCLR increase the range of backgrounds that do not impact the representation.


% This is going to be integrated into previous parts
% ***
% \subsection{ME: Augmenting SimCLR with time-constrastive information}

% We observe that our SimCLR-TT approach can reach similar performance to classic SimCLR and supervised learning on the validation set. For randomwalk views our results show a steady increase of performance with the number of fixations, which is expected. When comparing both view sampling approaches the uniform views especially help in generalizing to unseen frames from the same distribution.  However, the SimCLR-TT approach struggles to generalize seen objects to an unseen object of the same category on its own, as seen in Figure 6B. The generalization are only comparable with the supervised approach. Note that the uniform sampling (orange) does better than the randomwalk (blue), which is consistent with our experiments regarding object rotation in the house-environment.
% Augmenting the standard SimCLR approach with time-contrastive information substantially improves the generalization capabilities of the trained networks (dashed lines), by revealing information about the 3D structure of objects and placing the same object within different backgrounds. We also did an ablation on different values for the frequency of session changes and indicate peak performance with a star, cf. Appendix \ref{sec:sessionchanges}, \figref{fig:N06}.

\rebut{Moreover}, we analysed the frequency of session changes compared to the duration of object manipulations as one of the hyperparameters of our approach \rebut{in the CORe50 Environment, see Figure \figref{fig:persession_ablation}C, D}. Qualitatively, for \rebut{category classification} we observe \rebut{low accuracies for} \rebut{high-frequency object switches}, low session changes \rebut{and high accuracies for} \rebut{low-frequency object switches}, high session changes. Accuracy seems to more or less saturate at the main diagonal. \rebut{We infer from this that} intermediate values may actually be better than going to the extreme, but \rebut{it} could also be partly because  $N_{s}$ is bounded by $N_{o}$. The classification of sessions consistently shows that session information is being disregarded when the frequency of session changes rises.

%However, even at the lowest setting, around 50~\% of the session information is still retained.

%% 
% \subsection{ME: Discussion}
% % Why do I think the experiments turned out as they did?
% \begin{enumerate}
%     \item Time-based augmentations provide crucial information to generalize to the overarching category of objects
%     \item Session changes and number of fixations determine the approach
%     \item intermediate values might actually be better than going to the extreme, but generalization could also saturate at the main diagonal, because $N_{s}$ is limited by $N_{o}$
%     \item 
% \end{enumerate}
% ***


% \subsection{Color invariance matters}

\section{Conclusion}

% We investigated the impact of time-based, infant-inspired interactions with objects as a data-augmentation method on a representation learnt through CL. We studied these interactions through a real-world dataset of hand-based object manipulations in different environments and a novel 3D simulation environment where an agent ``plays'' with objects in a house. In both experiments, we find that combining time-based augmentations with conventional data-augmentations improves generalization over categories of objects. Our analysis shows that 1- object rotations are crucial to build shape-oriented categories; 2- Moving while holding object can prevent the background from cluttering the representation. We additionally validated our findings on a real-world video dataset and showed that time-based, natural augmentations provide crucial information to generalize to the overaching category of objects.

We investigated the \rebut{benefits} of time-based data-augmentations during infant-inspired natural object interactions \rebut{for self-supervised visual representation learning}. We studied these interactions through a novel 3-D simulation environment where an agent ``plays'' with objects in a house, and we validated our findings on two real-world video \rebut{datasets} of object manipulations. We find that combining time-based augmentations with conventional data-augmentations \rebut{(*-TT+ algorithms)} greatly improves the ability of the learned representations to generalize over object categories. Our analysis shows that 1) \rebut{3-D} object rotations are crucial to build good representations of shape categories. 2) Ego-motion while holding an object so that it is seen against different backgrounds prevents the background from cluttering the learned representation.
%We additionally validated our findings on a real-world video dataset and showed that time-based, natural augmentations provide crucial information to generalize to the overaching category of objects.
%and, in line with previous work \citep{wang2021use}, we highlighted that saccades can have a similar effect as random cropping. 

\rebut{Our work raises the question whether time-based augmentations during natural interactions with objects could fully replace conventional ones. Indeed, we showed that 3-D rotations are superior to the flip data-augmentation for shape generalization (\appref{sec:flip}). However, we found that color-based transformations like color jittering and grayscaling remain important. It is an interesting question for future work if time-based augmentations during changes of direct and indirect lighting or shadows cast by other objects could replace augmentations based on simple image color manipulations.}

%of lighting could simulate this in a time-contrastive approach, the TDW platform does not support ray-tracing, which would allow modeling such illumination changes realistically. 

%Other ideas of limitation: no realistic manipulation and no hand in TDW, small core50 dataset
Our work has a number of limitations. First, while we have portrayed the time-based augmentations as stemming from object {\em manipulations}, we did not render a hand holding the object or similar in the VHE and 3DShapeE. Second, the CORe50 and ToyBox environments are \rebut{only medium-sized}. Large scale experiments may give additional insights.
%, but require a fundamental change of learning paradigm towards embodied agents that interact with realistic environments.
Finally, in this work, we only considered naive behavioural strategies for, e.g., turning objects or ego-motion. This contrasts with the way infants learn about their environment \citep{bambach2016active}. For example, they are biased towards creating planar views of objects and often prefer unfamiliar objects \citep{roder2000infants}. Thus, we expect that learning to actively select successive views will further unveil the potential of time-based augmentations. 
%\citep{pereira2010early}, synchronize their saccades and focus distance according to the fixation point 

 % Large scale experiments may require a fundamental change of paradigm in self-supervised learning
%Experiments on larger dataset with richer and more controlled forms of object manipulations may provide additional insights.
%In addition, the hand should be apparent \cite{yu2009active}, we do not display it in TDW and leave to future works to establish how it relates to occlusion-based augmentations \cite{fong2019occlusions,zhong2020random}.


% restate main results
% draw some comparisons between rate of rotation <-> randomwalking
% draw some comparison between room-changes <-> session changes
% discuss why rotation rate is proportional to category accuracy, but inversely related to object accuracy. ME: I still think it has to do with learning invariances that are specific to the object rather than the category. Think of mugs, some have a handle, some don't, but if you only slowly rotate you might identify the handle as a specific feature of a mug, whereas the overall convex shape that can hold liquid is the determining feature 
%AR: fully agree with that

%  hand and leave to future works its impact on the learnt representations and its relations with occlusion-based data-augmentations.
%  While in practice, the observers' hand should be apparent \cite{yu2009active}, for the sake of simplicity, we do not display it.

\section*{Acknowledgements}
%This work was sponsored by a public grant overseen by the French National Agency through the IMobS3 Laboratory of Excellence (ANR-10-LABX-0016) and the IDEX-ISITE initiative CAP 20-25 (ANR-16-IDEX-0001). Financial support was also received from Clermont Auvergne Metropole through a French Tech-Clermont Auvergne professorship. We gratefully acknowledge support from the CNRS/IN2P3 Computing Center (Lyon - France) for providing computing and data-processing resources needed for this work. This work was also performed using HPC resources from GENCI–IDRIS (Grant 2022-AD011011623R1). JT was supported by the Johanna Quandt foundation. 
Removed for double-blind review.
% un-comment for the final submission not needed for double-blind review process
% 
% @Arthur you should probably put something in regarding cluster usage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Object manipulations and egomotion are crucial for category recognition}
%The relative performance of standard data-augmentations with respect to time-based augmentations is less evident. 

% Here, we want to the importance of the data-augmentations and compare SimCLR-TT with standard data-augmentations. 
%We omit the saccade augmentation and leave its analysis to \secref{app:saccades}. We 
%First, we observe that all SimCLR augmentations are at least not hurting the representation and at best, improving it. %We also observe that modifying the distance of the object is generally beneficial for the representation. 

% In \figref{fig:bigexp}A, we compare several variants of SimCLR-TT against SimCLR and a combination of both in the VHE. Baseline for comparison is SimCLR with its standard augmentations (black curve). %Adding frequent room changes (purple curve) does not affect performance. The green (rot(30)+D+Ns=2) variant simulates an infant that plays in one room, turns regularly, slowly rotates objects, brings them closer/farther and use SimCLR augmentations. The blue curve (rot(360)+D+Ro+Ns=1) displays an extreme case of a simulated infant that always changes rooms while very quickly rotating objects. In red (rot(360)+D+Ro+Ns=1+SimCLR), we observe the same extreme case, but combined with SimCLR augmentations. We clearly see that the best variant of SimCLR-TT outperforms SimCLR by a large margin and that both can be combined to further increase the overall performance. 


% For the CORe50 Environment we observe that the SimCLR-TT approach can outperform conventional SimCLR and supervised learning on the validation set. For random walk view sampling \figref{fig:bigexp}C shows a steady increase of performance with the number of fixations, which is expected. When comparing both view sampling approaches the uniform view sampling especially helps in generalizing to unseen video frames featuring the same sessions and objects as the training data, i.e., the validation set.  However, the SimCLR-TT approach struggles to generalize seen objects to an unseen object of the same category on its own, as seen in \figref{fig:bigexp}D. The generalization capabilities do not exceed the conventional SimCLR approach. Note that the uniform sampling (orange) does perform better than the random walk (blue), which is consistent with our experiments regarding object rotation in the VHE.  Combining the standard SimCLR augmentations with time-contrastive augmentations substantially improves the generalization capabilities (dashed curves). We also did an ablation on different values for the frequency of session changes,
% %and indicate peak performance with a star,
% cf.\ appendix~\ref{sec:sessionchanges}.

% For the ToyBox environment, we observe that the combination of SimCLR and SimCLR-TT substantially improves the accuracy when using both one composed augmentation per sample (TJGCBH, One aug) and one augmentation per sample per training step (TJGCBH). Color jittering is crucial to benefit from time-based augmentations (TJ versus T). We presume SimCLR-TT over-encodes the lighting conditions in Toybox and in the CORe-50 environment. However this is not an issue in the VHE where we ensure the background is strictly independent from the objects.

% Overall, combining the standard SimCLR augmentations with time-contrastive augmentations substantially improves the generalization capabilities by revealing information about the 3D structure of objects and placing the same object within different backgrounds. In the next sections, we analyze the impact of rotations and motion speed on the learnt representations. For other augmentation methods, in the Appendix, we emphasize the contribution of each time-based and conventional augmentation for category recognition. We also discuss how saccades relate to the conventional crop/resize data-augmentation in the \appref{app:abla_syne}.
%Show SimCLR-TT, SimCLR-TT + jitter + grayscale
%Show Core50 transformations versus simclr
% Show SimCLR-TT + simclr, SimCLR-TT, simclr, SimCLR-TT + jitter + gray

==> Time To Augment Contrastive Learning – ICLR23/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

